Parametric schedulability analysis of a launcher flight control system under reactivity constraints

The next generation of space systems will have to achieve more and more complex missions. In order to master the development cost and duration of such systems, an alternative to a manual design is to automatically synthesize the main parameters of the system. In this paper, we present an approach on the specific case of the scheduling of the flight control of a space launcher. The approach requires two successive steps: (1) the formalization of the problem to be solved in a parametric formal model and (2) the synthesis of the model parameters with a tool. We first describe the problematic of the scheduling of a launcher flight control, then we show how this problematic can be formalized with parametric stopwatch automata; we then present the results computed by IMITATOR. We compare the results to the ones obtained by other tools classically used in scheduling.

==> figures/reactivityNCC-useless.tex <==
\begin{tikzpicture}[scale=1.3, auto, ->, >=stealth']

	\node[location, initial] at (0,0) (init) [align=center] {\styleloc{init}};
	% Invariant
% 	\node [invariant, above] at (init.north) {\begin{tabular}{@{} c @{\ } c@{} }& $ \styleclock{xT1} \leq \styleparam{offsetT1}$\\\end{tabular}};

	\node[location] at (2, 0) (execNav) [align=center] {\styleloc{exec\_N}};
	% Invariant
% 	\node [invariant,above] at (execNav.north) {\begin{tabular}{@{} c @{\ } c@{} }& $ \styleclock{xT1} \leq \deadlineTone{}$ \\ $\land$ & $ \styleclock{xExecN} \leq \styleparam{WCETN}$ \end{tabular}};

	\node[location] at (4, 0) (finNav) [align=center] {\styleloc{finished\_N}};
	% Invariant
% 	\node [invariant,above] at (execNav.north) {\begin{tabular}{@{} c @{\ } c@{} }& $ \styleclock{xT1} \leq \deadlineTone{}$ \\ $\land$ & $ \styleclock{xExecN} \leq \styleparam{WCETN}$ \end{tabular}};

	\node[location] at (6, 0) (waitG) [align=center] {\styleloc{wait\_G}};

	\node[location] at (8, 0) (execG) [align=center] {\styleloc{exec\_G}};

	\node[location] at (8, -1) (finG) [align=center] {\styleloc{finished\_G}};

	\node[location] at (8, -2) (waitC) [align=center] {\styleloc{wait\_C}};

	\node[location] at (6, -2) (execC) [align=center] {\styleloc{exec\_C}};

	\node[location] at (4, -2) (waitG') [align=center] {\styleloc{finished\_C}};

	\node[location] at (2, -2) (good) [align=center] {\styleloc{good}};

	\node[location] at (4, -1) (bad) [align=center] {\styleloc{bad}};

% 	\path (init) edge node[above]{\begin{tabular}{@{} c @{\ } c@{} }
% 	& $\styleclock{xT1} = \styleparam{offsetT1}$\\
% % 		 & $\styleact{actControl}$\\
% 		& $\styleclock{xT1}:=0$\\
% 	\end{tabular}} (execNav);

	\path (init) edge node[above]{\styleact{startN}} node[below]{$\styleclock{xNGC} := 0$} (execNav);
	\path (init) edge[loop above] node[above]{\styleact{\Actions_{NGC}}} (init);

	\path (execNav) edge node[auto]{\styleact{finishN}} (finNav);
	\path (execNav) edge[loop above] node[above]{\allActExcept{\styleact{finishN}}} (execNav);
	
	\path (finNav) edge node[auto]{\styleact{finishT1 NOOO}} (waitG);
	\path (finNav) edge[loop above] node[above]{\allActExcept{\styleact{finishT1}}} (finNav);
	
	\path (waitG) edge node[auto]{\styleact{startG}} (execG);
	\path (waitG) edge[loop above] node[above]{\allActExcept{\styleact{startG}}} (waitG);
	
	\path (execG) edge node[auto]{\styleact{finishG}} (finG);
	\path (execG) edge[loop above] node[above]{\allActExcept{\styleact{finishG}}} (execG);
	
	\path (finG) edge node[auto]{\styleact{finishT2 NOOO}} (waitC);
	\path (finG) edge[loop right] node[right]{\allActExcept{\styleact{finishT2}}} (finG);
	
	\path (waitC) edge node[auto]{\styleact{startC}} (execC);
	\path (waitC) edge[loop right] node[right]{\allActExcept{\styleact{startC}}} (waitC);
	
	\path (execC) edge node[auto]{\styleact{finishC}} (waitG');
	\path (execC) edge[loop below] node[right]{\allActExcept{\styleact{finishC}}} (execC);
	
	\path (waitG') edge node[auto]{\styleact{finishT1 NOOO}} (good);
	\path (waitG') edge[loop below] node[right]{\allActExcept{\styleact{finishT1}}} (waitG');
	
	\path (waitG') edge node[auto]{\styleact{finishT1}} (bad);
\end{tikzpicture}

